Onboard Real-Time Multi-Sensor Pose Estimation for Indoor Quadrotor Navigation with Intermittent Communication

We propose a multisensor fusion framework for onboard real-time navigation of a quadrotor in an indoor environment, by integrating sensor readings from an Inertial Measurement Unit (IMU), a camera-based object detection algorithm, and an Ultra-WideBand (UWB) localization system. The sensor readings from the camera-based object detection algorithm and the UWB localization system arrive intermittently, since the measurements are not readily available. We design a Kalman filter that manages intermittent observations in order to handle and fuse the readings and estimate the pose of the quadrotor for tracking a predefined trajectory. The system is implemented via a Hardware-in-the-loop (HIL) simulation technique, in which the dynamic model of the quadrotor is simulated in an open-source 3D robotics simulator tool, and the whole navigation system is implemented on Artificial Intelligence (AI) enabled edge GPU. The simulation results show that our proposed framework offers low positioning and trajectory errors, while handling intermittent sensor measurements.

==> bibliography_archive.tex <==
\begin{thebibliography}{00}
\bibitem{2018:Chli} R. Mascaro, L. Teixeira, and T. Hinzmann, and R. Siegwart, and M. Chli, ``GOMSF: Graph-optimization based multi-sensor fusion for robust UAV pose estimation,'' in 2018 IEEE International Conference on Robotics and Automation (ICRA), 2018, pp. 1421–1428.

\bibitem{preiss2017crazyswarm} J. A. Preiss, W. Honig, G. S. Sukhatme, and N. Ayanian, “Crazyswarm: A large nano-quadcopter swarm,” in IEEE International Conference on Robotics and Automation (ICRA), 2017, pp. 3299–3304.

\bibitem{sa2018dynamic} I. Sa, M. Kamel, R. Khanna, M. Popovic, J. Nieto, and R. Siegwart, “Dynamic system identification, and control for a cost-effective and open-source multi-rotor mav,” in Springer Field and Service Robotics, 2018, pp. 605–620.

\bibitem{ghadiok2011autonomous} V. Ghadiok, J. Goldin, and W. Ren, “Autonomous indoor aerial gripping using a quadrotor,” in IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), 2011, pp. 4645–4651.

\bibitem{weiss2012real} S. Weiss, M. W. Achtelik, S. Lynen, M. Chli, and R. Siegwart, “Realtime onboard visual-inertial state estimation and self-calibration of mavs in unknown environments,” in IEEE International Conference on Robotics and Automation (ICRA), 2012, pp. 957–964.

%\bibitem{lim2015monocular} H. Lim and S. N. Sinha, “Monocular localization of a moving person onboard a quadrotor mav,” in IEEE International Conference on Robotics and Automation (ICRA), 2015, pp. 2182–2189.

%\bibitem{agrawal2006real} M. Agrawal and K. Konolige, “Real-time localization in outdoor environments using stereo vision and inexpensive gps,” in 18th International conference on pattern recognition (ICPR’06), vol. 3. IEEE, 2006, pp. 1063–1068.

\bibitem{garcia20043d} M. A. Garcia and A. Solanas, “3d simultaneous localization and modeling from stereo vision,” in IEEE International Conference on Robotics and Automation, 2004. Proceedings. ICRA’04. 2004, vol. 1. IEEE, 2004, pp. 847–853.

\bibitem{fraundorfer2012vision} F. Fraundorfer, L. Heng, D. Honegger, G. H. Lee, L. Meier, P. Tanskanen, and M. Pollefeys, “Vision-based autonomous mapping and exploration using a quadrotor mav,” in 2012 IEEE/RSJ International Conference on Intelligent Robots and Systems. IEEE, 2012, pp. 4557–4564.

\bibitem{maffra2019real} F. Maffra, L. Teixeira, Z. Chen, and M. Chli, “Real-time wide-baseline place recognition using depth completion,” IEEE Robotics and Automation Letters, vol. 4, no. 2, pp. 1525–1532, 2019.

\bibitem{ledergerber2015robot} A. Ledergerber, M. Hamer, and R. D’Andrea, “A robot self-localization system using one-way ultra-wideband communication,” in IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), 2015, pp. 3131–3137.

\bibitem{tiemann2017scalable} J. Tiemann and C. Wietfeld, “Scalable and precise multi-uav indoor navigation using tdoa-based uwb localization,” in IEEE International Conference on Indoor Positioning and Indoor Navigation (IPIN), 2017, pp. 1–7.

%\bibitem{papastratis2018indoor} I. Papastratis, T. Charalambous, and N. Pappas, “Indoor navigation of quadrotors via ultra-wideband wireless technology,” in Advances in Wireless and Optical Communications (RTUWO), 2018, pp. 106–111.

% \bibitem{garcia2019convolutional} A. Garcia, S. S. Mittal, E. Kiewra, and K. Ghose, “A convolutional neural network vision system approach to indoor autonomous quadrotor navigation,” in IEEE International Conference on Unmanned Aircraft Systems (ICUAS), 2019, pp. 1344–1352.

\bibitem{garcia2016indoor} S. García, M. E. López, R. Barea, L. M. Bergasa, A. Gómez, and E. J. Molinos, “Indoor slam for micro aerial vehicles control using monocular camera and sensor fusion,” in IEEE International Conference on Autonomous Robot Systems and Competitions (ICARSC), 2016, pp. 205–210.

\bibitem{bavle2018stereo} H. Bavle, S. Manthe, P. de la Puente, A. Rodriguez-Ramos, C. Sampedro, and P. Campoy, “Stereo visual odometry and semantics based localization of aerial robots in indoor environments,” in IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS). IEEE, 2018, pp. 1018–1023.

\bibitem{redmon2016you} J. Redmon, S. Divvala, R. Girshick, and A. Farhadi, “You only look once: Unified, real-time object detection, ”in Proceedings of the IEEE conference on computer vision and pattern recognition, 2016, pp. 779–788.

% \bibitem{jung2018perception} S. Jung, S. Hwang, H. Shin, and D. H. Shim, “Perception, guidance, and navigation for indoor autonomous drone racing using deep learning,” IEEE Robotics and Automation Letters, vol. 3, no. 3, pp. 2539–2544, 2018.

\bibitem{kendoul2006nonlinear} F. Kendoul, D. Lara, I. Fantoni, and R. Lozano, “Nonlinear Control for Systems with Bounded Inputs: Real-Time Embedded Control Applied to UAVs, ” in IEEE Conference on Decision and Control (CDC), 2006,pp. 5888–5893.

%\bibitem{voos2009nonlinear} H. Voos, “Nonlinear Control of a Quadrotor micro-UAV using Feedback-Linearization, ”in IEEE International Conference on Mechatronics, 2009, pp. 1–6.

\bibitem{sabatino2015quadrotor} F. Sabatino, “Quadrotor control: modeling, nonlinear control design, and simulation,” 2015.

\bibitem{bouabdallah2007design} S. Bouabdallah, “Design and Control of Quadrotors with Application to Autonomous Flying, ”Ecole Polytechnique Fédérale de Lausanne(EPFL), Tech. Rep., 2007.



% \bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
% \bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
% \bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
% \bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
% \bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
% \bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
% \bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.

\end{thebibliography}

==> figures/hil.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp622742387934] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.15 ] (340,55) -- (435,55) -- (435,110) -- (340,110) -- cycle ;
%Shape: Cloud [id:dp14132453399904465] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.1 ][dash pattern={on 2.25pt off 0.75pt}] (224.64,74.68) .. controls (223.8,69.85) and (226.58,65.07) .. (231.8,62.37) .. controls (237.02,59.67) and (243.77,59.53) .. (249.17,62) .. controls (251.09,59.19) and (254.6,57.26) .. (258.64,56.78) .. controls (262.68,56.3) and (266.77,57.33) .. (269.68,59.57) .. controls (271.32,57.03) and (274.53,55.32) .. (278.17,55.05) .. controls (281.81,54.79) and (285.37,56.01) .. (287.58,58.27) .. controls (290.54,55.58) and (295.23,54.44) .. (299.64,55.37) .. controls (304.04,56.29) and (307.36,59.1) .. (308.17,62.59) .. controls (311.78,63.36) and (314.79,65.32) .. (316.41,67.95) .. controls (318.04,70.58) and (318.12,73.63) .. (316.64,76.31) .. controls (320.2,79.92) and (321.03,84.72) .. (318.82,88.92) .. controls (316.61,93.13) and (311.69,96.1) .. (305.91,96.74) .. controls (305.86,100.69) and (303.08,104.31) .. (298.62,106.2) .. controls (294.16,108.1) and (288.74,107.98) .. (284.43,105.88) .. controls (282.59,110.61) and (277.41,114.08) .. (271.15,114.8) .. controls (264.88,115.52) and (258.64,113.36) .. (255.12,109.24) .. controls (250.8,111.26) and (245.62,111.84) .. (240.75,110.84) .. controls (235.88,109.85) and (231.72,107.36) .. (229.22,103.95) .. controls (224.81,104.35) and (220.55,102.56) .. (218.55,99.48) .. controls (216.55,96.41) and (217.25,92.69) .. (220.28,90.18) .. controls (216.35,88.37) and (214.35,84.8) .. (215.32,81.31) .. controls (216.29,77.83) and (220.01,75.23) .. (224.55,74.87) ; \draw  [dash pattern={on 2.25pt off 0.75pt}] (220.28,90.18) .. controls (222.14,91.03) and (224.28,91.42) .. (226.43,91.29)(229.22,103.95) .. controls (230.15,103.87) and (231.05,103.69) .. (231.91,103.42)(255.12,109.24) .. controls (254.47,108.49) and (253.93,107.67) .. (253.5,106.83)(284.43,105.88) .. controls (284.76,105.02) and (284.98,104.13) .. (285.08,103.23)(305.91,96.74) .. controls (305.96,92.54) and (302.89,88.68) .. (298.03,86.83)(316.64,76.31) .. controls (315.85,77.74) and (314.65,79.01) .. (313.13,80.01)(308.17,62.59) .. controls (308.3,63.17) and (308.36,63.76) .. (308.35,64.34)(287.58,58.27) .. controls (286.85,58.95) and (286.24,59.7) .. (285.78,60.51)(269.68,59.57) .. controls (269.29,60.18) and (269,60.83) .. (268.81,61.5)(249.17,62) .. controls (250.32,62.52) and (251.38,63.15) .. (252.32,63.87)(224.64,74.68) .. controls (224.75,75.35) and (224.94,76.01) .. (225.18,76.65) ;
%Shape: Rectangle [id:dp33265624971326957] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.15 ] (130,55) -- (195,55) -- (195,110) -- (130,110) -- cycle ;
%Straight Lines [id:da864901180462388] 
\draw    (320,70) -- (337,70) ;
\draw [shift={(340,70)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da2945875595831261] 
\draw    (195,70) -- (220,70) ;
%Straight Lines [id:da9954198959255367] 
\draw    (310,95) -- (340,95) ;
%Straight Lines [id:da5383827957984066] 
\draw    (215,95) -- (198,95) ;
\draw [shift={(195,95)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da17733988454045269] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (215,95) -- (310,95) ;
%Straight Lines [id:da1386604624207599] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (220,70) -- (320,70) ;

% Text Node
\draw (162.5,82.5) node   [align=left] {\begin{minipage}[lt]{44.2pt}\setlength\topsep{0pt}
\begin{center}
{\small Quadrotor Dynamics}\\{\small (Gazebo)}
\end{center}

\end{minipage}};
% Text Node
\draw (387.5,82.5) node   [align=left] {\begin{minipage}[lt]{64.43pt}\setlength\topsep{0pt}
\begin{center}
{\small Control System (ROS Node on NVIDIA Jetson)}
\end{center}

\end{minipage}};
% Text Node
\draw (282.5,82) node   [align=left] {\begin{minipage}[lt]{78.2pt}\setlength\topsep{0pt}
{\small ROS messages}
\end{minipage}};
% Text Node
\draw (272.5,45) node   [align=left] {\begin{minipage}[lt]{98.6pt}\setlength\topsep{0pt}
{\small Communication Network}
\end{minipage}};


\end{tikzpicture}


==> figures/system_architecture.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,362); %set diagram left start at 0, and has height of 362

%Rounded Rect [id:dp7251841161561732] 
\draw  [fill={rgb, 255:red, 245; green, 245; blue, 245 }  ,fill opacity=1 ] (82.67,120.2) .. controls (82.67,104.07) and (95.74,91) .. (111.87,91) -- (199.47,91) .. controls (215.59,91) and (228.67,104.07) .. (228.67,120.2) -- (228.67,239.13) .. controls (228.67,255.26) and (215.59,268.33) .. (199.47,268.33) -- (111.87,268.33) .. controls (95.74,268.33) and (82.67,255.26) .. (82.67,239.13) -- cycle ;
%Rounded Rect [id:dp42758928921648276] 
\draw  [fill={rgb, 255:red, 245; green, 245; blue, 245 }  ,fill opacity=1 ] (264.63,126.08) .. controls (264.63,106.39) and (280.59,90.42) .. (300.29,90.42) -- (422.83,90.42) .. controls (442.53,90.42) and (458.5,106.39) .. (458.5,126.08) -- (458.5,233.08) .. controls (458.5,252.78) and (442.53,268.75) .. (422.83,268.75) -- (300.29,268.75) .. controls (280.59,268.75) and (264.63,252.78) .. (264.63,233.08) -- cycle ;
%Rounded Rect [id:dp20959996762995803] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (87.67,128.13) .. controls (87.67,119.78) and (94.44,113) .. (102.8,113) -- (148.2,113) .. controls (156.56,113) and (163.33,119.78) .. (163.33,128.13) -- (163.33,247.2) .. controls (163.33,255.56) and (156.56,262.33) .. (148.2,262.33) -- (102.8,262.33) .. controls (94.44,262.33) and (87.67,255.56) .. (87.67,247.2) -- cycle ;
%Rounded Rect [id:dp7390349844751118] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (95.33,145.13) .. controls (95.33,140.83) and (98.83,137.33) .. (103.13,137.33) -- (145.2,137.33) .. controls (149.51,137.33) and (153,140.83) .. (153,145.13) -- (153,168.53) .. controls (153,172.84) and (149.51,176.33) .. (145.2,176.33) -- (103.13,176.33) .. controls (98.83,176.33) and (95.33,172.84) .. (95.33,168.53) -- cycle ;
%Rounded Rect [id:dp9976461626817317] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (95.33,192.87) .. controls (95.33,186.5) and (100.5,181.33) .. (106.87,181.33) -- (141.47,181.33) .. controls (147.84,181.33) and (153,186.5) .. (153,192.87) -- (153,245.8) .. controls (153,252.17) and (147.84,257.33) .. (141.47,257.33) -- (106.87,257.33) .. controls (100.5,257.33) and (95.33,252.17) .. (95.33,245.8) -- cycle ;
%Rounded Rect [id:dp7283164374580091] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (104.57,157.67) .. controls (104.57,156.19) and (105.76,155) .. (107.23,155) -- (142.17,155) .. controls (143.64,155) and (144.83,156.19) .. (144.83,157.67) -- (144.83,165.67) .. controls (144.83,167.14) and (143.64,168.33) .. (142.17,168.33) -- (107.23,168.33) .. controls (105.76,168.33) and (104.57,167.14) .. (104.57,165.67) -- cycle ;
%Rounded Rect [id:dp7937552119658933] 
\draw  [fill={rgb, 255:red, 225; green, 213; blue, 231 }  ,fill opacity=1 ] (172.9,133.67) .. controls (172.9,131.27) and (174.84,129.33) .. (177.23,129.33) -- (217.67,129.33) .. controls (220.06,129.33) and (222,131.27) .. (222,133.67) -- (222,146.67) .. controls (222,149.06) and (220.06,151) .. (217.67,151) -- (177.23,151) .. controls (174.84,151) and (172.9,149.06) .. (172.9,146.67) -- cycle ;
%Rounded Rect [id:dp801148736999107] 
\draw  [fill={rgb, 255:red, 248; green, 206; blue, 204 }  ,fill opacity=1 ] (104.9,202.33) .. controls (104.9,200.86) and (106.09,199.67) .. (107.57,199.67) -- (142.5,199.67) .. controls (143.97,199.67) and (145.17,200.86) .. (145.17,202.33) -- (145.17,210.33) .. controls (145.17,211.81) and (143.97,213) .. (142.5,213) -- (107.57,213) .. controls (106.09,213) and (104.9,211.81) .. (104.9,210.33) -- cycle ;
%Rounded Rect [id:dp906278769068829] 
\draw  [fill={rgb, 255:red, 225; green, 213; blue, 231 }  ,fill opacity=1 ] (105.57,221.67) .. controls (105.57,220.19) and (106.76,219) .. (108.23,219) -- (143.17,219) .. controls (144.64,219) and (145.83,220.19) .. (145.83,221.67) -- (145.83,229.67) .. controls (145.83,231.14) and (144.64,232.33) .. (143.17,232.33) -- (108.23,232.33) .. controls (106.76,232.33) and (105.57,231.14) .. (105.57,229.67) -- cycle ;
%Rounded Rect [id:dp9722291040628013] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (105.23,240.67) .. controls (105.23,239.19) and (106.43,238) .. (107.9,238) -- (142.83,238) .. controls (144.31,238) and (145.5,239.19) .. (145.5,240.67) -- (145.5,248.67) .. controls (145.5,250.14) and (144.31,251.33) .. (142.83,251.33) -- (107.9,251.33) .. controls (106.43,251.33) and (105.23,250.14) .. (105.23,248.67) -- cycle ;
%Rounded Rect [id:dp4936985256866846] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (171.57,240) .. controls (171.57,237.61) and (173.51,235.67) .. (175.9,235.67) -- (216.33,235.67) .. controls (218.73,235.67) and (220.67,237.61) .. (220.67,240) -- (220.67,253) .. controls (220.67,255.39) and (218.73,257.33) .. (216.33,257.33) -- (175.9,257.33) .. controls (173.51,257.33) and (171.57,255.39) .. (171.57,253) -- cycle ;
%Straight Lines [id:da4381351376242979] 
\draw    (172,245.5) -- (147.75,245.5) ;
\draw [shift={(144.75,245.5)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Rounded Rect [id:dp7087074484390583] 
\draw  [fill={rgb, 255:red, 245; green, 245; blue, 245 }  ,fill opacity=1 ] (376.88,155.03) .. controls (376.88,146.45) and (383.83,139.5) .. (392.4,139.5) -- (438.98,139.5) .. controls (447.55,139.5) and (454.5,146.45) .. (454.5,155.03) -- (454.5,223.98) .. controls (454.5,232.55) and (447.55,239.5) .. (438.98,239.5) -- (392.4,239.5) .. controls (383.83,239.5) and (376.88,232.55) .. (376.88,223.98) -- cycle ;
%Rounded Rect [id:dp44272261265042934] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (383.5,192.67) .. controls (383.5,191.19) and (384.69,190) .. (386.17,190) -- (445.33,190) .. controls (446.81,190) and (448,191.19) .. (448,192.67) -- (448,200.67) .. controls (448,202.14) and (446.81,203.33) .. (445.33,203.33) -- (386.17,203.33) .. controls (384.69,203.33) and (383.5,202.14) .. (383.5,200.67) -- cycle ;
%Rounded Rect [id:dp619262226491538] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (383.5,219.67) .. controls (383.5,218.19) and (384.69,217) .. (386.17,217) -- (445.33,217) .. controls (446.81,217) and (448,218.19) .. (448,219.67) -- (448,227.67) .. controls (448,229.14) and (446.81,230.33) .. (445.33,230.33) -- (386.17,230.33) .. controls (384.69,230.33) and (383.5,229.14) .. (383.5,227.67) -- cycle ;
%Rounded Rect [id:dp3336214918166853] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=1 ] (383.5,166.67) .. controls (383.5,165.19) and (384.69,164) .. (386.17,164) -- (445.33,164) .. controls (446.81,164) and (448,165.19) .. (448,166.67) -- (448,174.67) .. controls (448,176.14) and (446.81,177.33) .. (445.33,177.33) -- (386.17,177.33) .. controls (384.69,177.33) and (383.5,176.14) .. (383.5,174.67) -- cycle ;
%Rounded Rect [id:dp42314496733127416] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (284,166.67) .. controls (284,165.19) and (285.19,164) .. (286.67,164) -- (342.83,164) .. controls (344.31,164) and (345.5,165.19) .. (345.5,166.67) -- (345.5,174.67) .. controls (345.5,176.14) and (344.31,177.33) .. (342.83,177.33) -- (286.67,177.33) .. controls (285.19,177.33) and (284,176.14) .. (284,174.67) -- cycle ;
%Rounded Rect [id:dp6127406845584862] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (283.5,141.17) .. controls (283.5,139.69) and (284.69,138.5) .. (286.17,138.5) -- (307.33,138.5) .. controls (308.81,138.5) and (310,139.69) .. (310,141.17) -- (310,149.17) .. controls (310,150.64) and (308.81,151.83) .. (307.33,151.83) -- (286.17,151.83) .. controls (284.69,151.83) and (283.5,150.64) .. (283.5,149.17) -- cycle ;
%Rounded Rect [id:dp29542307836523474] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (318,141.92) .. controls (318,140.44) and (319.19,139.25) .. (320.67,139.25) -- (341.83,139.25) .. controls (343.31,139.25) and (344.5,140.44) .. (344.5,141.92) -- (344.5,149.92) .. controls (344.5,151.39) and (343.31,152.58) .. (341.83,152.58) -- (320.67,152.58) .. controls (319.19,152.58) and (318,151.39) .. (318,149.92) -- cycle ;
%Rounded Rect [id:dp3242092521343509] 
\draw  [fill={rgb, 255:red, 245; green, 245; blue, 245 }  ,fill opacity=1 ] (279,216.37) .. controls (279,212.76) and (281.93,209.83) .. (285.53,209.83) -- (345.47,209.83) .. controls (349.07,209.83) and (352,212.76) .. (352,216.37) -- (352,235.97) .. controls (352,239.57) and (349.07,242.5) .. (345.47,242.5) -- (285.53,242.5) .. controls (281.93,242.5) and (279,239.57) .. (279,235.97) -- cycle ;
%Rounded Rect [id:dp042292598769395395] 
\draw  [fill={rgb, 255:red, 213; green, 232; blue, 212 }  ,fill opacity=1 ] (100.82,284.33) .. controls (100.82,282.31) and (102.46,280.67) .. (104.48,280.67) -- (143.33,280.67) .. controls (145.36,280.67) and (147,282.31) .. (147,284.33) -- (147,295.33) .. controls (147,297.36) and (145.36,299) .. (143.33,299) -- (104.48,299) .. controls (102.46,299) and (100.82,297.36) .. (100.82,295.33) -- cycle ;
%Straight Lines [id:da025550693063846275] 
\draw    (124.38,250.75) -- (124.26,277.5) ;
\draw [shift={(124.25,280.5)}, rotate = 270.24] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da3306298384087314] 
\draw    (146.38,226.25) -- (276.38,226.01) ;
\draw [shift={(279.38,226)}, rotate = 539.89] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da43011128061443316] 
\draw    (183,216.75) -- (276,216.38) ;
\draw [shift={(279,216.37)}, rotate = 539.77] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da8385826002653649] 
\draw    (183,216.75) -- (183.13,206) ;
%Straight Lines [id:da4393011041364012] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (164.13,206.5) -- (174.13,206.5) ;
%Straight Lines [id:da08900870914748293] 
\draw    (144.88,207) -- (161.88,206.75) ;
%Straight Lines [id:da08697488387132846] 
\draw    (243.88,162) -- (147.75,162.24) ;
\draw [shift={(144.75,162.25)}, rotate = 359.86] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da21203411813966855] 
\draw    (173,140.25) -- (167.13,140.25) ;
%Straight Lines [id:da9393281282561545] 
\draw    (167.13,140.25) -- (167.38,155.25) ;
%Straight Lines [id:da2368360693423024] 
\draw    (175.88,206) -- (183.13,206) ;
%Straight Lines [id:da687498007888947] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (167.38,157.25) -- (167.63,167.5) ;
%Straight Lines [id:da5858379717413784] 
\draw    (167.63,170.25) -- (167.63,221.5) ;
%Straight Lines [id:da29807585888293264] 
\draw    (167.63,221.5) -- (148.83,221.64) ;
\draw [shift={(145.83,221.67)}, rotate = 359.56] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da5678230919267313] 
\draw    (146.63,289.25) -- (244.38,288.75) ;
%Straight Lines [id:da5873776617674937] 
\draw    (244.38,235.5) -- (244.38,288.75) ;
%Straight Lines [id:da18278774056386804] 
\draw    (244.38,235.5) -- (276.13,235.5) ;
\draw [shift={(279.13,235.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da33118944459623445] 
\draw    (243.88,162) -- (243.88,197) ;
%Straight Lines [id:da7652563746577425] 
\draw    (383.63,197.5) -- (243.88,197) ;
%Straight Lines [id:da42746259888594684] 
\draw    (296.63,151.75) -- (296.63,161) ;
\draw [shift={(296.63,164)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da8404335632729547] 
\draw    (331.13,152.25) -- (331.13,161.5) ;
\draw [shift={(331.13,164.5)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da7321861641315295] 
\draw    (345.88,171.25) -- (381.13,171.25) ;
\draw [shift={(384.13,171.25)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da09377680449865622] 
\draw    (314.88,242.75) -- (314.88,255) ;
%Straight Lines [id:da8573234952204147] 
\draw    (417.13,255.5) -- (314.88,255) ;
%Straight Lines [id:da7922551805928191] 
\draw    (417.13,255.5) -- (417.13,234.5) ;
\draw [shift={(417.13,231.5)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Straight Lines [id:da8324661693852955] 
\draw    (366,207) -- (366,255.25) ;
%Straight Lines [id:da8306955899105231] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (365.88,193.75) -- (366.13,204) ;
%Straight Lines [id:da13133391236339453] 
\draw    (366.13,190.75) -- (311.88,190.5) ;
%Straight Lines [id:da356667114153272] 
\draw    (311.88,190.5) -- (311.88,180.75) ;
\draw [shift={(311.88,177.75)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;
%Curve Lines [id:da012086319690592706] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (90.5,287.7) .. controls (89.63,309) and (92.63,309) .. (120.63,307.75) ;
%Straight Lines [id:da24718027483799698] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (122.63,307.75) -- (432.38,308) ;
%Curve Lines [id:da9535388944133798] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435.63,308.25) .. controls (449.38,308) and (464.63,313) .. (465.38,288.5) ;
%Straight Lines [id:da2206100027837039] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (464.4,99.4) -- (465.38,286) ;
%Curve Lines [id:da937657739954117] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (433.63,80.5) .. controls (471.13,78.5) and (463.88,82.75) .. (464.63,96.5) ;
%Straight Lines [id:da40227443231493676] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (430.38,80.9) -- (270.63,80.4) ;
%Curve Lines [id:da5829752328667539] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (90.38,285) .. controls (88.88,266) and (97.38,271.75) .. (105.63,271) ;
%Straight Lines [id:da6694092030791634] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (105.63,271) -- (206.13,269.75) ;
%Curve Lines [id:da15688426823273738] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (208.88,269.75) .. controls (221.88,268.5) and (234.63,274.75) .. (235.13,251.25) ;
%Straight Lines [id:da16032606036362917] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (234,99) -- (235.13,251.25) ;
%Curve Lines [id:da21254664022563685] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (234.33,94.65) .. controls (232.83,75.65) and (259.58,81.15) .. (267.83,80.4) ;

% Text Node
\draw (113.67,94) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Gazebo Simulator}};
% Text Node
\draw (89.33,120) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize DJI M100 (UAV)}};
% Text Node
\draw (104.13,139.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Actuators}};
% Text Node
\draw (106.27,183.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Sensors}};
% Text Node
\draw (178.7,133.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Anchors}};
% Text Node
\draw (179.9,239.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Objects}};
% Text Node
\draw (116.37,199) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize IMU}};
% Text Node
\draw (113.7,219.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize UWB}};
% Text Node
\draw (107.03,238.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Camera}};
% Text Node
\draw (109.7,155.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Motors}};
% Text Node
\draw (338.1,102.6) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize ROS Nodes}};
% Text Node
\draw (397.5,142) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize LQ-Servo}};
% Text Node
\draw (405,164) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Path}};
% Text Node
\draw (384,189.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Control Vector}};
% Text Node
\draw (404.5,217.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize State}};
% Text Node
\draw (289,164) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Path Planer}};
% Text Node
\draw (285.5,138) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Goal}};
% Text Node
\draw (321.25,138.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Map}};
% Text Node
\draw (280.5,212) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{49.13pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Estimator}\\{\footnotesize (Sensor Fusion)}
\end{center}

\end{minipage}};
% Text Node
\draw (109.9,283.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize YOLO}};
% Text Node
\draw (315.5,252.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize State}};
% Text Node
\draw (363.85,249.55) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-269.54] [align=left] {{\footnotesize Pose}};
% Text Node
\draw (324.25,277.75) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Jetson AGX Xavier}};


\end{tikzpicture}


==> figures/system_block_diagram_final.tex <==
%%% for the head arrow size search for this ->  (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.86pt,y=0.80pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,669); %set diagram left start at 0, and has height of 669

%Straight Lines [id:da9357914636873921] 
\draw    (715,253.5) -- (715,285.5) ;
%Rounded Rect [id:dp3660675060067178] 
\draw  [fill={rgb, 255:red, 245; green, 245; blue, 245 }  ,fill opacity=1 ] (40.62,276.38) .. controls (40.62,275.07) and (41.69,274) .. (43,274) -- (169.29,274) .. controls (170.6,274) and (171.67,275.07) .. (171.67,276.38) -- (171.67,425.62) .. controls (171.67,426.93) and (170.6,428) .. (169.29,428) -- (43,428) .. controls (41.69,428) and (40.62,426.93) .. (40.62,425.62) -- cycle ;
%Rounded Rect [id:dp10502667026891799] 
\draw  [fill={rgb, 255:red, 218; green, 232; blue, 252 }  ,fill opacity=0.2 ] (44,299.57) .. controls (44,297.6) and (45.6,296) .. (47.57,296) -- (114.43,296) .. controls (116.4,296) and (118,297.6) .. (118,299.57) -- (118,420.43) .. controls (118,422.4) and (116.4,424) .. (114.43,424) -- (47.57,424) .. controls (45.6,424) and (44,422.4) .. (44,420.43) -- cycle ;
%Rounded Rect [id:dp7523000327490585] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (50,317) .. controls (50,315.34) and (51.34,314) .. (53,314) -- (109,314) .. controls (110.66,314) and (112,315.34) .. (112,317) -- (112,342) .. controls (112,343.66) and (110.66,345) .. (109,345) -- (53,345) .. controls (51.34,345) and (50,343.66) .. (50,342) -- cycle ;
%Rounded Rect [id:dp7632193787189323] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (50,354.6) .. controls (50,353.16) and (51.16,352) .. (52.6,352) -- (109.4,352) .. controls (110.84,352) and (112,353.16) .. (112,354.6) -- (112,418.4) .. controls (112,419.84) and (110.84,421) .. (109.4,421) -- (52.6,421) .. controls (51.16,421) and (50,419.84) .. (50,418.4) -- cycle ;
%Rounded Rect [id:dp9871651402160917] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.2 ] (54,328.8) .. controls (54,327.25) and (55.25,326) .. (56.8,326) -- (101.2,326) .. controls (102.75,326) and (104,327.25) .. (104,328.8) -- (104,337.2) .. controls (104,338.75) and (102.75,340) .. (101.2,340) -- (56.8,340) .. controls (55.25,340) and (54,338.75) .. (54,337.2) -- cycle ;
%Rounded Rect [id:dp46280925486877567] 
\draw  [fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.2 ] (54,368.8) .. controls (54,367.25) and (55.25,366) .. (56.8,366) -- (101.2,366) .. controls (102.75,366) and (104,367.25) .. (104,368.8) -- (104,377.2) .. controls (104,378.75) and (102.75,380) .. (101.2,380) -- (56.8,380) .. controls (55.25,380) and (54,378.75) .. (54,377.2) -- cycle ;
%Rounded Rect [id:dp20874533365343995] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.2 ] (54,386.8) .. controls (54,385.25) and (55.25,384) .. (56.8,384) -- (101.2,384) .. controls (102.75,384) and (104,385.25) .. (104,386.8) -- (104,395.2) .. controls (104,396.75) and (102.75,398) .. (101.2,398) -- (56.8,398) .. controls (55.25,398) and (54,396.75) .. (54,395.2) -- cycle ;
%Rounded Rect [id:dp05307079608726628] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.2 ] (54,404.8) .. controls (54,403.25) and (55.25,402) .. (56.8,402) -- (101.2,402) .. controls (102.75,402) and (104,403.25) .. (104,404.8) -- (104,413.2) .. controls (104,414.75) and (102.75,416) .. (101.2,416) -- (56.8,416) .. controls (55.25,416) and (54,414.75) .. (54,413.2) -- cycle ;
%Rounded Rect [id:dp9326668104709761] 
\draw  [fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.2 ] (122,348.8) .. controls (122,347.25) and (123.25,346) .. (124.8,346) -- (163.2,346) .. controls (164.75,346) and (166,347.25) .. (166,348.8) -- (166,357.2) .. controls (166,358.75) and (164.75,360) .. (163.2,360) -- (124.8,360) .. controls (123.25,360) and (122,358.75) .. (122,357.2) -- cycle ;
%Rounded Rect [id:dp1536768733841889] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.2 ] (122,404.8) .. controls (122,403.25) and (123.25,402) .. (124.8,402) -- (163.2,402) .. controls (164.75,402) and (166,403.25) .. (166,404.8) -- (166,413.2) .. controls (166,414.75) and (164.75,416) .. (163.2,416) -- (124.8,416) .. controls (123.25,416) and (122,414.75) .. (122,413.2) -- cycle ;
%Straight Lines [id:da30984959969959647] 
\draw    (122.5,410) -- (107,410) ;
\draw [shift={(104,410)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Straight Lines [id:da5254658405623513] 
\draw    (144,370) -- (107,370) ;
\draw [shift={(104,370)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Rounded Rect [id:dp34398873207599046] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.2 ] (60,440.8) .. controls (60,439.25) and (61.25,438) .. (62.8,438) -- (97.2,438) .. controls (98.75,438) and (100,439.25) .. (100,440.8) -- (100,449.2) .. controls (100,450.75) and (98.75,452) .. (97.2,452) -- (62.8,452) .. controls (61.25,452) and (60,450.75) .. (60,449.2) -- cycle ;
%Straight Lines [id:da6745155360782911] 
\draw    (80,416) -- (80,435) ;
\draw [shift={(80,438)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Rounded Rect [id:dp7593076326055295] 
\draw  [fill={rgb, 255:red, 245; green, 245; blue, 245 }  ,fill opacity=1 ] (178,293.4) .. controls (178,291.52) and (179.52,290) .. (181.4,290) -- (306.6,290) .. controls (308.48,290) and (310,291.52) .. (310,293.4) -- (310,424.6) .. controls (310,426.48) and (308.48,428) .. (306.6,428) -- (181.4,428) .. controls (179.52,428) and (178,426.48) .. (178,424.6) -- cycle ;
%Rounded Rect [id:dp4319447534259082] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.2 ] (186,367.29) .. controls (186,365.47) and (187.47,364) .. (189.29,364) -- (232.71,364) .. controls (234.53,364) and (236,365.47) .. (236,367.29) -- (236,414.71) .. controls (236,416.53) and (234.53,418) .. (232.71,418) -- (189.29,418) .. controls (187.47,418) and (186,416.53) .. (186,414.71) -- cycle ;
%Straight Lines [id:da8246435513610142] 
\draw    (104,392) -- (183,392) ;
\draw [shift={(186,392)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Straight Lines [id:da6669034809869188] 
\draw    (100,446) -- (174,446) ;
%Straight Lines [id:da7461930640913232] 
\draw    (144,360) -- (144,370) ;
%Straight Lines [id:da7507238292148792] 
\draw    (104,374) -- (183,374) ;
\draw [shift={(186,374)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Straight Lines [id:da044351333584915276] 
\draw    (174,410) -- (174,446) ;
%Straight Lines [id:da9395917315652298] 
\draw    (174,410) -- (183,410) ;
\draw [shift={(186,410)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Straight Lines [id:da8737127874571562] 
\draw    (107,332) -- (190,332) ;
\draw [shift={(104,332)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Rounded Rect [id:dp1482883222547109] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.2 ] (244,308.8) .. controls (244,307.25) and (245.25,306) .. (246.8,306) -- (301.2,306) .. controls (302.75,306) and (304,307.25) .. (304,308.8) -- (304,317.2) .. controls (304,318.75) and (302.75,320) .. (301.2,320) -- (246.8,320) .. controls (245.25,320) and (244,318.75) .. (244,317.2) -- cycle ;
%Straight Lines [id:da06793408921650079] 
\draw    (274,392) -- (236,392) ;
%Rounded Rect [id:dp6840363076452589] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.2 ] (244,332.8) .. controls (244,331.25) and (245.25,330) .. (246.8,330) -- (267.2,330) .. controls (268.75,330) and (270,331.25) .. (270,332.8) -- (270,341.2) .. controls (270,342.75) and (268.75,344) .. (267.2,344) -- (246.8,344) .. controls (245.25,344) and (244,342.75) .. (244,341.2) -- cycle ;
%Straight Lines [id:da622890058646159] 
\draw    (244,312) -- (233,312) ;
\draw [shift={(230,312)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Rounded Rect [id:dp2260648512692096] 
\draw  [fill={rgb, 255:red, 139; green, 87; blue, 42 }  ,fill opacity=0.2 ] (186,298.38) .. controls (186,296.4) and (187.6,294.8) .. (189.58,294.8) -- (234.42,294.8) .. controls (236.4,294.8) and (238,296.4) .. (238,298.38) -- (238,356.42) .. controls (238,358.4) and (236.4,360) .. (234.42,360) -- (189.58,360) .. controls (187.6,360) and (186,358.4) .. (186,356.42) -- cycle ;
%Rounded Rect [id:dp4159887705849614] 
\draw  [fill={rgb, 255:red, 139; green, 87; blue, 42 }  ,fill opacity=0.2 ] (190,308.8) .. controls (190,307.25) and (191.25,306) .. (192.8,306) -- (227.2,306) .. controls (228.75,306) and (230,307.25) .. (230,308.8) -- (230,317.2) .. controls (230,318.75) and (228.75,320) .. (227.2,320) -- (192.8,320) .. controls (191.25,320) and (190,318.75) .. (190,317.2) -- cycle ;
%Rounded Rect [id:dp06340448387420317] 
\draw  [fill={rgb, 255:red, 139; green, 87; blue, 42 }  ,fill opacity=0.2 ] (190,326.8) .. controls (190,325.25) and (191.25,324) .. (192.8,324) -- (227.2,324) .. controls (228.75,324) and (230,325.25) .. (230,326.8) -- (230,335.2) .. controls (230,336.75) and (228.75,338) .. (227.2,338) -- (192.8,338) .. controls (191.25,338) and (190,336.75) .. (190,335.2) -- cycle ;
%Rounded Rect [id:dp8630554823205185] 
\draw  [fill={rgb, 255:red, 139; green, 87; blue, 42 }  ,fill opacity=0.2 ] (190,344.8) .. controls (190,343.25) and (191.25,342) .. (192.8,342) -- (227.2,342) .. controls (228.75,342) and (230,343.25) .. (230,344.8) -- (230,353.2) .. controls (230,354.75) and (228.75,356) .. (227.2,356) -- (192.8,356) .. controls (191.25,356) and (190,354.75) .. (190,353.2) -- cycle ;
%Rounded Rect [id:dp42117947472795225] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.2 ] (278,332.8) .. controls (278,331.25) and (279.25,330) .. (280.8,330) -- (301.2,330) .. controls (302.75,330) and (304,331.25) .. (304,332.8) -- (304,341.2) .. controls (304,342.75) and (302.75,344) .. (301.2,344) -- (280.8,344) .. controls (279.25,344) and (278,342.75) .. (278,341.2) -- cycle ;
%Straight Lines [id:da21578990269496834] 
\draw    (256,323) -- (256,330) ;
\draw [shift={(256,320)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Straight Lines [id:da9512074346199] 
\draw    (290,323) -- (290,330) ;
\draw [shift={(290,320)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Straight Lines [id:da03271049395289882] 
\draw    (274,323) -- (274,392) ;
\draw [shift={(274,320)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Flowchart: Connector [id:dp11406092940595047] 
\draw   (273,350) .. controls (273,349.45) and (273.45,349) .. (274,349) .. controls (274.55,349) and (275,349.45) .. (275,350) .. controls (275,350.55) and (274.55,351) .. (274,351) .. controls (273.45,351) and (273,350.55) .. (273,350) -- cycle ;
%Straight Lines [id:da8543443686925141] 
\draw    (273,350) -- (233,350) ;
\draw [shift={(230,350)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (4.57,-2.72) -- (0,0) -- (4.57,2.72) -- cycle    ;
%Shape: Polygon [id:ds1627597140696866] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (316,274) -- (316,454) -- (40,454) -- (40,432) -- (174,432) -- (174,274) -- cycle ;

% Text Node
\draw (65,276) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Gazebo Simulator}};
% Text Node
\draw (46,298) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize DJI M100 (UAV)}};
% Text Node
\draw (59,315) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Actuators}};
% Text Node
\draw (65,329) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Motors}};
% Text Node
\draw (63,354) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Sensors}};
% Text Node
\draw (67,369) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize UWB}};
% Text Node
\draw (69,387) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize IMU}};
% Text Node
\draw (63,405) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Camera}};
% Text Node
\draw (128,404) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Objects}};
% Text Node
\draw (127,348) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Anchors}};
% Text Node
\draw (66,441) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize YOLO}};
% Text Node
\draw (191,374) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{30.29pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Estimator}
\end{center}

\end{minipage}};
% Text Node
\draw (248,412) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize ROS Nodes}};
% Text Node
\draw (196,390) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{23.41pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Sensor}
\end{center}

\end{minipage}};
% Text Node
\draw (197,400) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{22.32pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Fusion}
\end{center}

\end{minipage}};
% Text Node
\draw (185,295) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{35.66pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize LQ-Servo}
\end{center}

\end{minipage}};
% Text Node
\draw (201,308) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Path}};
% Text Node
\draw (196,326) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Control}};
% Text Node
\draw (201,344) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize State}};
% Text Node
\draw (247,308) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Path Planner}};
% Text Node
\draw (246,332) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Goal}};
% Text Node
\draw (281,332) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Map}};
% Text Node
\draw (247,378) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Pose}};
% Text Node
\draw (203,436) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\footnotesize Jetson AGX Xavier}};


\end{tikzpicture}


==> results/results.tex <==
% \documentclass{article}

% \usepackage{pgfplots, pgfplotstable}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsfonts}
% \usepackage{graphicx}

\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{shapes,arrows,calc,spy}
\pgfplotsset{grid style={dashed}}

% \thispagestyle{empty}
% \begin{document}


\begin{figure}[t!]
% \centering
\begin{center}

\begin{tikzpicture}
\begin{axis}
% [height=3.5cm,
% width=10cm,
[height=5.5cm,
width=9.4cm,
legend style={font=\footnotesize},
legend columns={-1},
% legend pos=north, % This was causing an error, and it doesn't seem to affect the output. So i commented it out.
legend cell align={left}, 
smooth,
point meta=explicit,
ylabel shift = 0pt,
%cycle list={{blue},{dashed}},
minor tick num=1,
ylabel style={yshift=-0.4cm},
axis equal=false,
line width=0.7pt,
no markers,
grid=major,
grid style={dashed,black!50},        % but don't show the grid or the tick for the `extra ticks'
        extra x tick style={
        grid=none,
        major tick length=0pt,},
x label style={at={(axis description cs:0.5,0)}},
y label style={at={(axis description cs:0,0.5)}},
%xmajorgrids,
%ymajorgrids,
 axis on top,
xmin=0,
xmax=20,
ymin=-2.5,
ymax=2.5,
xlabel=position - $x$~(m),ylabel=position - $y$~(m)]
% xmin=0,
% xmax=60,
% ymin=0,
% ymax=4,
% xlabel=position - $x$~(m),ylabel=position - $y$~(m)]


% \addplot+[blue] table [x expr=\thisrowno{0}/20, y=x9, col sep=comma] {states.csv};
% Desired path
\addplot+[dashed, black] table [x=Desired X, y=Desired Y, col sep=comma] {results/imu_uwb_path_following.csv};
% IMU & UWB
\addplot+[blue] table [x=Actual X, y=Actual Y, col sep=comma] {results/imu_uwb_path_following.csv};
% Sensor Fusion
\addplot+[red] table [x=Actual X, y=Actual Y, col sep=comma] {results/sensor_fusion_path_following.csv};

\addlegendentry{Goal}
\addlegendentry{IMU \& UWB}
\addlegendentry{IMU \& UWB \& YOLO}


%% For background color
% \addplot+[domain=0:20,samples=2,name path=A,black,forget plot] {0};
% \addplot+[domain=0:20,samples=2,name path=B,black,forget plot] {10};
% \addplot[blue!5] fill between[of=A and B];
% \addlegendentry{IMU}
% \addplot+[domain=20:40,samples=2,name path=C,black,forget plot] {0};
% \addplot+[domain=20:40,samples=2,name path=D,black,forget plot] {10};
% \addplot[blue!15] fill between[of=C and D];
% \addlegendentry{IMU+YOLO}
% \addplot+[domain=40:60,samples=2,name path=E,black,forget plot] {0};
% \addplot+[domain=40:60,samples=2,name path=F,black,forget plot] {10};
% \addplot[blue!25] fill between[of=E and F];
% \addlegendentry{IMU+YOLO+UWB}
\end{axis}
%\spy[size=2cm,magnification=3] on (4,1) in node at (4,-1);
\end{tikzpicture}


\label{fig:example_of_a_trajectory}
\end{center}
\vspace{-0.5cm}\caption{Example of a trajectory.}
\end{figure}







